Favi-Score: A Measure for Favoritism in Automated Preference Ratings for Generative AI Evaluation

Generative AI systems have become ubiquitous for all kinds of modalities, which makes the issue of the evaluation of such models more pressing. One popular approach is preference ratings, where the generated outputs of different systems are shown to evaluators who choose their preferences. In recent years the field shifted towards the development of automated (trained) metrics to assess generated outputs, which can be used to create preference ratings automatically. In this work, we investigate the evaluation of the metrics themselves, which currently rely on measuring the correlation to human judgments or computing sign accuracy scores. These measures only assess how well the metric agrees with the human ratings. However, our research shows that this does not tell the whole story. Most metrics exhibit a disagreement with human system assessments which is often skewed in favor of particular text generation systems, exposing a degree of favoritism in automated metrics. This paper introduces a formal definition of favoritism in preference metrics, and derives the Favi-Score, which measures this phenomenon. In particular we show that favoritism is strongly related to errors in final system rankings. Thus, we propose that preference-based metrics ought to be evaluated on both sign accuracy scores and favoritism.

==> algo/phi.tex <==
\begin{algorithm}[!t]
\small
\caption{Computation of Favi-Score} 
\label{algo:faviscore}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}


\Input{Generative Systems $\pi_a, \pi_b$}
\Input{Preference Ratings $\mathcal{R}^H$ and $\mathcal{R}^A$}
\Input{Testset $\mathcal{T} \subseteq \mathcal{I}$}
\Output{Favoritism Score $\Phi$}

\Begin{


let $C \in \mathbb{N}^{3 \times 3}$ : Confusion Matrix

let $d \in \mathbb{N}^{3}$ : Outcome Counts according to $\mathcal{R}^H$

initialize C and d with zeros

define $idx : \{$ + : 0, = : 1, - : 2 $\}$ %\to \{1, 2, 3\}$ with $index(+) = 1, index(=) = 2, index(-) = 3$

\ForEach {test sample $t \in \mathcal{T}$}{
    $r^H = \mathcal{R}^H(\pi_a(t), \pi_b(t))$ the preference rating according to $\mathcal{R}^H$ of the outputs of $\pi_a$ and $\pi_b$ for test sample $t$
    
    $r^A = \mathcal{R}^A(\pi_a(t), \pi_b(t))$

    increase $C_{idx[r^A], idx[r^H]}$ by 1

    increase $d_{idx[r^H]}$ by 1
}
let $\mu \in \mathbb{R}^{3 \times 3}$: Mixture Matrix

$\mu_{ij} = \frac{C_ij}{ \sum_{k=1}^3 C_{kj}}$ for $i, j = 1..3$

let $p \in \mathbb{R}^{3}$ : Outcome Distribution  

$p_i = \frac{d_i}{\sum_{k=1}^3 d_k}$ for $i = 1..3$


$\Phi = \frac{1}{2}(p_1(-\mu_{2,1} -  2\mu_{3,1}) + p_2(\mu_{1,2} - \mu_{3,2}) + p_{3}(2\mu_{1,3}  + \mu_{2,3}))$


\Return $\Phi$;
}

\end{algorithm}

%\todo{in phi.tex: maybe add a caption to the algorithm and move the "index" function into the caption and explain that this just maps between the outcomes and the matrix indices.}

==> algo/phi_old.tex <==
\begin{algorithm}[!t]
\small
\caption{Fa$\Phi$-Score for system-pair} %using Error-prone Metrics}
\label{algo:faviscore}

\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\SetKwData{confmat}{Confusion Matrix}
\SetKwData{outcome}{True Outcome Counts}
\SetKwFunction{colnorm}{ColumnNormalize}
\SetKwFunction{lowtri}{LowerTriangle}
\SetKwFunction{upptri}{UpperTriangle}

\Input{$\pi_a, \pi_b$: Generative Systems}
\Input{$\mathcal{R}^H \in \{+, =, -\}$ human preference rating}
\Input{$\mathcal{R}^A \in \{+, =, -\}$ auto preference rating}
\Input{$\mathcal{T}$ test set}
\Output{Fa$\Phi$ Score}

\Begin{


$C \in \mathbb{N}^{3 \times 3}:$ \confmat;

$d \in \mathbb{N}^{3}:$ \outcome;

\ForEach{$i \in \mathcal{T}$}{
    $r^H[i] = \mathcal{R}^H(\pi_a(i), \pi_b(i))$
    
    $r^A[i] = \mathcal{R}^A(\pi_a(i), \pi_b(i))$
    
    $C[r^A[i], r^H[i]] += 1$

    $d[r^H[i]] += 1$
}
$\bm{\mu} = \colnorm(C)$ 

$\bm{p} =\colnorm(p)$ 

$f_1 = \upptri(\bm{\mu})p$

$f_2 = \lowtri(\bm{\mu})p$

$\Phi = \sum_{i=0}^2 (f_1 - f_2)[i]$


\Return $\Phi$;
}
\end{algorithm}

==> figures/all_box_plots.tex <==
\begin{figure*}[!t]
\small
\centering
\begin{subfigure}[c]{0.24\textwidth}
 \centering
     \includegraphics[width=0.9\textwidth]{figures/favi-plots//summeval_relevance_naive_pairwise_plot.pdf}
     \caption{SummEval Relevance}
     \label{fig:boxplot_summ_relevance}
 \end{subfigure}
 \begin{subfigure}[c]{0.24\textwidth}
 \centering
     \includegraphics[width=0.9\textwidth]{figures/favi-plots//summeval_coherence_naive_pairwise_plot.pdf}
     \caption{SummEval Coherence}
     \label{fig:boxplot_summ_coherence}
 \end{subfigure}
 \begin{subfigure}[c]{0.24\textwidth}
 \centering
     \includegraphics[width=0.9\textwidth]{figures/favi-plots/summeval_consistency_naive_pairwise_plot.pdf}
     \caption{SummEval Consistency}
     \label{fig:boxplot_summ_consistency}
 \end{subfigure}
 \begin{subfigure}[c]{0.24\textwidth}
 \centering
     \includegraphics[width=0.9\textwidth]{figures/favi-plots//summeval_fluency_naive_pairwise_plot.pdf}
     \caption{SummEval Fluency}
     \label{fig:boxplot_summ_fluency}
 \end{subfigure}
  \begin{subfigure}[c]{0.24\textwidth}
 \centering
     \includegraphics[width=0.9\textwidth]{figures/favi-plots//dialog_naive_pairwise_plot.pdf}
     \caption{Dialogue}
     \label{fig:boxplot_dialogue}
 \end{subfigure}
 \begin{subfigure}[c]{0.24\textwidth}
 \centering
     \includegraphics[width=0.9\textwidth]{figures/favi-plots//wmt21_naive_pairwise_plot.pdf}
     \caption{WMT21}
     \label{fig:boxplot_wmt}
 \end{subfigure}
  \begin{subfigure}[c]{0.24\textwidth}
 \centering
     \includegraphics[width=0.9\textwidth]{figures/favi-plots//wmt22_naive_pairwise_plot.pdf}
     \caption{WMT22}
     \label{fig:boxplot_wmt}
 \end{subfigure}
\caption{Visualization of the median (solid red) and mean (dashed purple) Unfairness Score with the corresponding box plots over each pair of TG systems. Note that the whiskers show the 5 and 95 percentiles, respectively.}
\label{fig:box_plots}
\end{figure*}



==> old_stuff.tex <==
\section{OLD}
\subsection{Absolute Symmetry}
Here, we prove lemma~\ref{lemm:symm}. 
\begin{lemma}[Symmetric]
    The absolute value of  Fa$\Phi$-Score is Symmetric. That is $|\Phi(\pi_a, \pi_b)| = |\Phi(\pi_b, \pi_a)|$.
\end{lemma}

First we note that the mixture matrix for $\mathcal{E}^{a,b}$ is given by:
\begin{equation}
    {\small
\begin{aligned}
    \bm{\mu}^{a,b} = 
    \begin{pmatrix}
        \mu_{++} & \mu_{+=} & \mu_{+-} \\
        \mu_{=+} & \mu_{==} & \mu_{=-} \\
        \mu_{-+} & \mu_{-=} & \mu_{--} \\
    \end{pmatrix}
    \end{aligned}}
\end{equation}

If we swap the systems, the values are rearranged as follows:

\begin{equation}
    {\small
\begin{aligned}
    \bm{\mu}^{b,a} = 
    \begin{pmatrix}
        \mu_{--} & \mu_{-=} & \mu_{-+} \\
        \mu_{=-} & \mu_{==} & \mu_{=+} \\
        \mu_{+-} & \mu_{+=} & \mu_{++} \\
    \end{pmatrix}
    \end{aligned}}
\end{equation}

Thus, the score changes to:

\begin{equation}
    {\small
\begin{aligned}
    f^1_{b,a} &= \begin{pmatrix}
       0 & \mu_{-=} & 2\mu_{-+} \\
        0 & 0 & \mu_{=+} \\
        0 & 0 & 0 \\
    \end{pmatrix}  \begin{pmatrix} p_- \\ p_= \\ p_+ \end{pmatrix} \\ 
    &= \begin{pmatrix} p_= \mu_{-=} + p_+ 2\mu_{-+} \\ p_+ \mu_{=+} \\ 0 \end{pmatrix} = f^2_{a,b}
    \end{aligned}}
\end{equation}

\begin{equation}
    {\small
\begin{aligned}
    f^2_{b,a} &= \begin{pmatrix}
        0 & 0 & 0 \\
        \mu_{=-} & 0 & 0 \\
        2\mu_{+-} & \mu_{+=} & 0 \\
    \end{pmatrix}  \begin{pmatrix} p_- \\ p_= \\ p_+ \end{pmatrix} \\ 
    &= \begin{pmatrix} 0 \\ p_- \mu_{=-} \\ p_-  2\mu_{+-} + p_=\mu_{+=} \end{pmatrix}= f^1_{a,b}
    \end{aligned}}
\end{equation}

Thus, we get that $\Phi(\pi_b, \pi_a)  = -\Phi(\pi_a, \pi_b)$ since $f_1$ and $f_2$ are swapped when the systems are swapped. Thus, the absolute values remain the same. 

\subsection{Fair implies no Sign Change} \label{app:no-sgn-change}
Here we show that if $\Phi = 0 \implies sgn(p_+ - p_-) = sng(\hat{p}_+ - \hat{p}_-)$. That means that under a fair metric, there are no changes in signs. More strictly, we even show that:

\begin{align}
\begin{split}
    &\Phi = 0 \implies  \\
    &\hat{p}_+ = p_+ + \frac{p_= - \hat{p}_=}{2}  \\
    & \land  \hat{p}_- = p_- + \frac{p_= - \hat{p}_=}{2}
    \end{split}
\end{align}

That is, the outcome is the same as if the ``='' were equally distributed. 

Let us first state the condition $\hat{p}_+ = p_+ + \frac{p_= - \hat{p}_=}{2}$ in terms of the linear transformation.
\begin{align}
\begin{split}
& \hat{p}_+ = p_+ + \frac{p_= - \hat{p}_=}{2} \\
&  \iff p_+ \mu_{++}  + p_= \mu_{+=} + p_- \mu_{+-}   \\
& = p_+ + \frac{p_= - p_+ \mu_{=+}  - p_= \mu_{==} - p_- \mu_{=-}}{2} \\
& \iff p_+ \mu_{++}  + p_= \mu_{+=} + p_- \mu_{+-} \\
& - p_+ - \frac{p_= - p_+ \mu_{=+}  - p_= \mu_{==} - p_- \mu_{=-}}{2}  = 0\\
& \iff p_+ \mu_{++}  + p_= \mu_{+=} + p_- \mu_{+-}\\
& - p_+ - \frac{p_=}{2} + \frac{p_+ \mu_{=+} }{2} + \frac{p_= \mu_{==}}{2} + \frac{p_- \mu_{=-}}{2} \\
& \iff 0 = p_+ (\mu_{++}  - 1 + \frac{\mu_{=+} }{2}) \\
& + p_= (\mu_{+=} - \frac{1}{2} + \frac{\mu_{==}}{2}) \\
& + p_- (\mu_{+-} + \frac{\mu_{=-}}{2}) \\
& \iff 0 = p_+ (- (1 - \mu_{++} ) + \frac{\mu_{=+} }{2}) \\
& + p_= (- \frac{1}{2}( 1- \mu_{+=})  + \frac{\mu_{+=}}{2}) \\
& + p_- (\mu_{+-} +  \frac{\mu_{=-}}{2}) \\
& \iff 0 = p_+ (- (\mu_{=+} + \mu_{-+} ) + \frac{\mu_{=+} }{2}) \\
& + p_= (- \frac{1}{2}( \mu_{+=} + \mu_{-=})  + \frac{\mu_{+=}}{2}) \\
& + p_- (\mu_{+-} + \frac{\mu_{=-}}{2}) \\
& \iff 0 = p_+ (- \frac{\mu_{=+} }{2}  - \mu_{-+}) \\
& + p_= (\frac{\mu_{+=}}{2} - \frac{\mu_{-=}}{2}) \\
& + p_- (\mu_{+-} + \frac{\mu_{=-}}{2}) = \Phi\\
\end{split}
\end{align}

Thus, we have shown that there is an equivalence of a fair metrics with $\Phi = 0$ and the outcome according to the metric, which is equivalent to an equal distribution of the ``=''. The derivation is analogous for $\hat{p}_- = p_- + \frac{p_= - \hat{p}_=}{2}$. This result implies that there is no possibility of a change in outcome/ranking under a fair metric. We also note that the equality only holds when we count the ``+''/ ``-'' confusions doubly. 

\section{Law of Total Probability} \label{app:law_of_total}
In this section, we prove lemma~\ref{lemma:lin_trafo}. For this we have to show that $\hat{\bm{p}} = \bm{\mu}\bm{p}$. First, we write the equation using all terms:

\begin{equation}
    {\small
\begin{aligned}
     \begin{pmatrix} \hat{p}_+ \\ \hat{p}_=\\ \hat{p}_- \end{pmatrix} = 
    \begin{pmatrix}
        \mu_{++} & \mu_{+=} & \mu_{+-} \\
        \mu_{=+} & \mu_{==} & \mu_{=-} \\
        \mu_{-+} & \mu_{-=} & \mu_{--} \\
    \end{pmatrix}  \begin{pmatrix} p_+ \\ p_= \\ p_- \end{pmatrix}
    \end{aligned}}
\end{equation}

Now we focus on one entry. Let $c \in \{+, =, -\}$.

\begin{equation}
    {\small
\begin{aligned}
     \hat{p}_c &= p_+*\mu_{c+} + p_=*\mu_{c=} + p_-*\mu_{c-} \\
     & = Pr(r^H[i] = \text{``+''})*Pr(r^A[i] =c | r^H[i] = \text{``+''}) \\
     & + Pr(r^H[i] = \text{``=''})*Pr(r^A[i] =c | r^H[i] = \text{``=''}) \\
     & + Pr(r^H[i] = \text{``-''})*Pr(r^A[i] =c | r^H[i] = \text{``-''}) \\
     & = \sum_{c' \in \{+, = , -\}} Pr(r^H[i] = c')*Pr(r^A[i] =c | r^H[i] = c') \\
     & = Pr(r^A[i] = c) = \hat{p}_c \qed
    \end{aligned}}
\end{equation}

Where the last line is the application of the law of total probability. 

\section{Favoritism Derivation} \label{app:derivation}

Here, we state the derivation of the favoritism score. The favoritism score analyses the direction in which the mistakes of a metric are skewed in contrast to the human ratings. That is, which percentage of the samples are disproportionately rated in favor of one system. The mistakes of a metric are denoted in the upper and lower triangle of the mixture matrix $\mu$. 

\begin{equation}
    {\small
\begin{aligned}
    \bm{\mu} = 
    \begin{pmatrix}
        \mu_{++} & \mu_{+=} & \mu_{+-} \\
        \mu_{=+} & \mu_{==} & \mu_{=-} \\
        \mu_{-+} & \mu_{-=} & \mu_{--} \\
    \end{pmatrix}
    \end{aligned}}
\end{equation}

The upper triangle of the matrix are the probabilities that a sample, which the humans rated either preferring system $\pi_2$ or as a draw being rated in disfavor of $\pi_2$. For instance $\mu_{+=}$ states the probability that if the humans rated a sample as a draw, that the metric rates it as preferring system $\pi_1$. The lower triangle of the mixture matrix are the probabilities that the metric rates samples in favor of $\pi_2$ compared to the human evaluations. 

Thus, if we observe an outcome distribution $\bm{p} = (p_+, p_=, p_-)^T$, the mixture matrix states the distribution that we can expect to observe under the metric $\hat{\bm{p}} = \bm{\mu}\bm{p}$. However, we are only interested in the mistakes, thus, we only consider the off-diagonal elements. Furthermore, we are interested in the mistakes in favor of the two systems. Thus, we consider the upper and lower triangle seperately, and then compute the difference. Thus, this yields the following derivaiton.


\begin{equation}
    {\small
\begin{aligned}
    f^1 &= \begin{pmatrix}
       0 & \mu_{+=} & 2\mu_{+-} \\
        0 & 0 & \mu_{=-} \\
        0 & 0 & 0 \\
    \end{pmatrix}  \begin{pmatrix} p_+ \\ p_= \\ p_- \end{pmatrix} \\ 
    &= \begin{pmatrix} p_= \mu_{+=} + p_- 2\mu_{+-} \\ p_- \mu_{=-} \\ 0 \end{pmatrix}
    \end{aligned}}
\end{equation}

\begin{equation}
    {\small
\begin{aligned}
    f^2 &= \begin{pmatrix}
        0 & 0 & 0 \\
        \mu_{=+} & 0 & 0 \\
        2\mu_{-+} & \mu_{-=} & 0 \\
    \end{pmatrix}  \begin{pmatrix} p_+ \\ p_= \\ p_- \end{pmatrix} \\ 
    &= \begin{pmatrix} 0 \\ p_+ \mu_{=+} \\ p_+  2\mu_{-+} + p_=\mu_{-=} \end{pmatrix}
    \end{aligned}}
\end{equation}

The entries in $f^1$ and $f^2$ denote the probability that a sample is treated favorably by the metric with regards to the human ratings. For instance: $p_= \mu_{+=} = Pr(r^H[i] = \text{``=''})*Pr(r^A[i] = \text{``+''} | r^H[i] = \text{``=''})$, which by application of Bayes' Rule equals $Pr(r^A[i] = \text{``+''} , r^H[i] = \text{``=''})$, i.e., the probability that the metric states ``+'' while the human rating states ``=''. Thus, the sum of all entries in $f_1$ equals the probability that a sample is rated in favor of $\pi_1$ according to the metric, while $f_2$ states the probability that a sample is rated in favor of $\pi_2$. 

In case where $\sum_i f^1_i = \sum_i f^2_i$, we speak of a fair metric, which does not favor one of the systems since the probability that samples are changed in favor of one system are balanced. Thus, in order to compute the favorability score, we take the difference: 

\begin{align}
    \small
    \begin{split}
        \Phi(\mathcal{E}) &= \frac{\sum_i f^1_i - \sum_i f^2_i}{2}\\ 
        &= \frac{1}{2}(p_+(-\mu_{=+} -  2\mu_{-+})  \\
        &+ p_=(\mu_{+=} - \mu_{-=}) \\
        & + p_{-}(2\mu_{+-}  + \mu_{=-}))
    \end{split} 
\end{align}

Thus, $\rho^{A}(\pi_1, \pi_2)$ states the percentage of samples that the metric changes too much in favor of one system. 

%\section{More Properties}
%First, we show that the absolute value Favi-Score is symmetric:%

%\begin{lemma}[Symmetric] \label{lemm:symm}
%    The absolute value of  Fa$\Phi$-Score is Symmetric. That is $|\Phi(\pi_a, \pi_b)| = |\Phi(\pi_b, \pi_a)|$. More precisely: $\Phi(\pi_b, \pi_a)  = -\Phi(\pi_a, \pi_b)$
%\end{lemma}

%That is, the sign of the Favi-Score changes when the systems are swapped, but the absolute value remains the same.

%The next property is that Favi-Score is not transitive:
%\begin{lemma}[Non-transitivity] \label{lemm:symm}
%    The value of  Fa$\Phi$-Score is non-transitive. That is $\Phi(\pi_a, \pi_b) > 0 \land \Phi(\pi_b, \pi_c) > 0 \centernot\implies \Phi(\pi_a, \pi_c) > 0$.
%\end{lemma}

%Thus, one has to compute the Fa$\Phi$-Score for each pair of systems, and it is not possible to infer $\Phi$ via transitivity. 

% Given $\mathcal{E}$, we now define the two outcome distributions according to the two preference ratings, $\mathcal{R}^H$ and  $\mathcal{R}^A$, respectively : 
% \begin{definition}[Outcome Distribution]
%     Given an evaluation setting $\mathcal{E}$ for preference ratings $\mathcal{R}^H$ and  $\mathcal{R}^A$, we define the \emph{Reference Pairwise Outcome Distribution} according for $\mathcal{R}^H$ as:
%     \begin{align}
%     \begin{split}
%          & \bm{p} = (p_{+}, p_{=}, p_{-})^T \\
%          & p_c = \frac{1}{|\mathcal{E}|}\sum_{i \in \mathcal{E}} \mathbb{I}[r[i], c] \\
%          & \forall c \in \{+, =, -\} 
%     \end{split}
%     \end{align}

%     The pairwise outcome distribution for the second preference rating $\mathcal{R}^A$ is defined analogously, and we denote it as $\hat{\bm{p}} = (\hat{p}_{+}, \hat{p}_{=}, \hat{p}_{-})^T$.
% \end{definition}

%  We interpret the outcome distribution as a probability distribution, thus, $p_+$ is interpreted as the probability that system $\pi_1$ generates an output preferred by the human ratings $\mathcal{R}^H$. We now  introduce the \emph{mixture matrix} to model the disagreement between the automated metric and the human preference ratings. 

% \begin{definition}[Mixture Matrix]
%     Given an evaluation setting $\mathcal{E}$,  we define the \emph{Mixture Matrix} $\mu$ as

%     \begin{equation}
%     {\small
%     \begin{aligned}
%         \bm{\mu} = 
%             \begin{pmatrix}
%             \mu_{++} & \mu_{+=} & \mu_{+-} \\
%             \mu_{=+} & \mu_{==} & \mu_{=-} \\
%             \mu_{-+} & 
%             \mu_{-=} & 
%             \mu_{--} \\
%         \end{pmatrix}
%     \end{aligned}}
% \end{equation}

% where each entry in the mixture matrix is defined as follows:    
%     \begin{equation}
% {\small
%         \begin{aligned}
%         \mu_{cc'} = \frac{\sum_{i \in \mathcal{E}} \mathbb{I}[r^A[i], c]*\mathbb{I}[r^H[i], c']}{\sum_{i \in \mathcal{E}} \mathbb{I}[r^H[i], c']}  \forall c, c'\in \{+, =, -\}
%         \end{aligned}}
%     \end{equation}
% \end{definition}

% Each entry in a mixture matrix can be interpreted as the following conditional probability:
% \begin{equation}
% {\small
%         \begin{aligned}
%         \mu_{cc'} = Pr(r^A[i] = c | r^H[i] = c')  \forall c, c'\in \{+, =, -\}
%         \end{aligned}}
% \end{equation}
% For instance, $\mu_{+=}$ states the probability that the automated metric prefers system $\pi_1$ over $\pi_2$ given that the humans do not have a preference. Note that each \emph{column} in the mixture matrix defines a probability distribution. %We will discuss the interpretation of $\bm{\mu}$ in the next section and how it relates to defining favoritism. 
% \paragraph{Example.} To make the notion of a mixture matrix clearer, consider the following example:
% \begin{equation}
% \label{eq:mu}
% \small
% \bm{\mu} = 
%         \begin{pmatrix}
%             0.6 & 0.2 & 0.3 \\
%             0.3 & 0.4 & 0.3 \\
%             0.1 & 0.4 & 0.4 \\
% \end{pmatrix}
% \end{equation}

% The first column tells us that a human rating $r^H[i] =\text{``+''}$ will be transformed into an automated rating $r^A[i] = \text{``+''}$ in 60\% of cases, $r^A[i] = \text{``=''}$ in 30\% of cases, and $r^A[i] = \text{``-''}$ in 10\% of cases. Thus, $\bm{\mu}$ is defined on the sample-level, which means that each column tells us what we expect how a human rating is transformed under the metric. This bring us to the following lemma:

% \begin{lemma}
% \label{lemma:lin_trafo}
%     There is a linear relation between $\bm{p}$ and $\hat{\bm{p}}$ described by $\bm{\mu}$. That is,
%     \begin{equation}
%         \hat{\bm{p}} = \bm{\mu}\bm{p}
%     \end{equation}
% \end{lemma}

% This lemma can be easily show via the Law of Total Probability (see Appendix~\ref{app:law_of_total}).

% %Before we turn to the definition of favoritism, we note the relationship between $\bm{p}$, and $\hat{\bm{p}}$ in terms of $\bm{\mu}$. It turns out that $\hat{\bm{p}} = \bm{\mu}\bm{p}$, which can be easily show via the Law of Total Probability (see Appendix~\ref{app:law_of_total}).

% \begin{table}[t!]
% \small
%  %\begin{subtable}{0.3\textwidth}
%     \centering
%     \include{tables/confusion_matrix}
%     %\end{subtable}
%     %\begin{subtable}{0.3\textwidth}
%     %\centering
%     %\include{tables/conf_mat_pm}
%     %\end{subtable}
%     %\begin{subtable}{0.3\textwidth}
%     %\centering
%     %\include{tables/conf_mat_em}
%     %\end{subtable}
%     \caption{Expected confusions according to the example $\mu$ from Equation~\ref{eq:mu}, when we observe 600 wins, 100 draws, and 300 losses according to human judgments (left). Each row shows how the samples are expected to be distributed according to the metric. The green cells show the number of samples that are distributed in favor of $\pi_2$, and the blue cells show the number of samples distributed in favor of $\pi_1$.}
%     \label{tab:expected_confusion}
% \end{table}

% \section{Favoritism Score}
% \label{sec:favi_def}
% We now define the notion of favoritism based on the formalism that we introduced in the previous section. First, we continue the example from the above section.  

% \paragraph{Example.} To understand the notion of favoritism, we investigate whether the differences between the human and metric ratings are systematically distributed in favor of one system. For this, assume that we collected an evaluation setting with 1000 samples $\mathcal{E}$ as in definition~\ref{def:eval_set}. For the sake of the example, we show the computation in terms of the raw counts instead of the probabilities. Assume that counting the preferences according to the human ratings we get that $\pi_1$ is preferred over $\pi_2$ 600 times, 100 times they have judge both outputs as equal quality (no preference), and in 300 cases, humans prefer $\pi_2$ over $\pi_1$. Furthermore, assume that the metric ratings prefer $\pi_1$ over $\pi_2$ 470 times, 310 times the metric judges them as equal, and in 220 cases it prefers $\pi_2$ over $\pi_1$. Finally, assume $\mu$ from Equation \ref{eq:mu}. 

% With this information, we can count how the metric distributes the ratings the confusion matrix is shown in Table~\ref{tab:expected_confusion}, left side. For instance the 600 ratings where the humans prefer  $\pi_1$ over $\pi_2$ are distributed by the metric in 360 times where the metric agrees with the human ratings, in 180 cases the metric rates those samples as equal, and in 60 cases it rates those samples as preferring $\pi_2$ over $\pi_1$ (this is a consequence of lemma~\ref{lemma:lin_trafo}).

% Now the question is: which system does this metric favor? From the outcomes themselves it is hard to judge, since in both cases system $\pi_1$ is overall still favored. However, the mistakes (highlighted in green and blue in Tablee~\ref{tab:expected_confusion}) are more indicative. The mistakes in the upper triangle (green) are the mistakes of the metric with regards to human judgments that are in favor of $\pi_2$, and those in the lower triangle (blue) are those mistakes that are in favor of $\pi_1$. In total, there are $280$ mistakes in favor of $\pi_2$ and 200 mistakes in favor of $\pi_1$. From this we can state that this metric disproportionately favors $\pi_2$ with 80 samples.

% However, the impact of the samples on the final outcome is not equal. In fact, the mistaking of a ``+'' with a ``-'' has double the impact than mistaking ``+'' with a ``=''. Since a  ``+''  $\leftrightarrow$ ``-'' mistake changes the gap between the samples in favor of $\pi_1$ to the number of samples in favor of $\pi_2$ by 2, while a  ``+''  $\leftrightarrow$ ``='' mistake  changes the gap by only 1. Thus the ``+'' $\leftrightarrow$ ``-'' mistakes needs to be counted double. This changes the examples as follows: the mistakes in the upper triangle have now a value of $180 + 2*60+40 = 340$, and the ones in the lower triangle $20 + 2*180 + 90 = 290$, thus the difference is now 50 in favor of $\pi_2$. This is plausible, since there are more confusions of ``+''  $\leftrightarrow$ ``-''  in favor of $\pi_1$ (90 vs. 60).

% %To illustrate this point, we slightly change the data and assume that there are 61 cases where the humans state it's a ``+'' but the metric states its a ``-'' (see Table~\ref{tab:expected_confusion} (middle)). Then by consequence, there are 359 cases where both agree on ``+''. In the outcome according to the metric there are now 469 times ``+'' and 221 times ``-'', which reduces the difference by 2. On the other hand, if we assume that the metric confuses ``='' with a ``-'' (see Table~\ref{tab:expected_confusion} (right)), the difference changes only by 1. Thus, the impact of the ``+'' $\leftrightarrow$ ``-'' confusions needs to be counted double. Thus, the mistakes in the upper triangle have now a value of $180 + 2*60+40 = 340$, and the ones in the lower triangle $20 + 2*180 + 90 = 290$, thus the difference is now 50 in favor of $\pi_2$. This is plausible, since there are more confusions of ``+''  $\leftrightarrow$ ``-''  in favor of $\pi_1$ (90 vs. 60).

% \paragraph{Formal Definition of Favoritism Score.} We are now ready to formalize our intuition of favoritism for two preference ratings:

% \begin{definition}[Favoritism Score (Favi-Score)]
% \label{def:faviscore}
%     Given an outcome $\bm{p}$ and a mixture matrix $\bm{\mu}$ computed on a fixed evaluation setting $\mathcal{E}$ for two preference ratings, we define the \emph{Favoritism Score$\Phi$} as:
%     \begin{align}
%     \small
%     \begin{split}
%     \Phi(\mathcal{E}) = \frac{1}{2}(&p_+(-\mu_{=+} -  2\mu_{-+})  \\
%     +& p_=(\mu_{+=} - \mu_{-=}) \\
%      + &p_{-}(2\mu_{+-}  + \mu_{=-}))
%     \end{split} 
% \end{align}
% \end{definition}
% Note that the fraction $\frac{1}{2}$ serves to limit the score between -1 and 1.

% %\begin{definition}[Fa$\Phi$-Score]
% %    Given an outcome $\bm{p}$ and a mixture matrix $\bm{\mu}$ computed on a fixed evaluation setting $\mathcal{E}$, we define the favoritism score as:
% %    \begin{align}
% %    \small
% %   \begin{split}
% %        \rho^{A}(\pi_1, \pi_2) &= p_+(-\mu_{=+} -  \mu_{-+})  \\
% %        &+ p_=(\mu_{+=} - \mu_{-=}) \\
% %        & + p_{-}(\mu_{+-}  + \mu_{=-})
% %    \end{split} 
% %\end{align}
% %Note that $\rho^{A}(\pi_1, \pi_2) \in [-1, 1]$
% %\end{definition}

% Put simply, the Favoritism Score is the result of multiplying the upper triangle of $\bm{\mu}$ with the outcome $\bm{p}$ and subtracting the multiplication of the lower triangle of $\bm{\mu}$ with the outcome $\bm{p}$, and then summing up. The sign of the score tells us in which direction the favoritism goes (positive towards $\pi_1$, negative towards $\pi_2$), and the magnitude tells us the percentage of samples that went disproportionately in favor of one system (see Appendix~\ref{app:derivation} for the full derivation). Since confusing a $+$ with a $-$ is more severe than confusing it with a $=$, we count the impact of  $\mu_{-+}$ and $\mu_{+-}$ doubly.

% %\begin{definition}[Final Fa$\Phi$-Score]
% %    Given an outcome $\bm{p}$ and a mixture matrix $\bm{\mu}$ computed on a fixed evaluation setting $\mathcal{E}$, we define the favoritism score as:
% %    \begin{align}
% %    \small
% %    \begin{split}
% %        \rho^{A}_{2}(\pi_1, \pi_2) &= \frac{1}{\beta}(p_+(-\mu_{=+} -  2\mu_{-+})  \\
% %        &+ p_=(\mu_{+=} - \mu_{-=}) \\
% %        & + p_{-}(2\mu_{+-}  + \mu_{=-}))
% %    \end{split} ,
% %\end{align},
% %where $\beta$ is a weight that states how much more severe we punish confusing a $+$ with a $-$. The faction $\frac{1}{\beta}$ serves to limit the score between -1 and 1.
% %\end{definition}

% %Usually, the naive value for $\beta = 2$, since confounding a ``+'' with a ``-'' costs double the amount than confusing a ``+'' with a ``=''. 

% To come back to our example, the Favi-Score score of our $\mu$ from Equation \ref{eq:mu} with  $\bm{p} = (0.6, 0.1, 0.3)^T$ is $\Phi(\mathcal{E}) = -0.05$, which matches the above example in Table Table~\ref{tab:expected_confusion}. 

% %\paragraph{Scope} Favoritism is a concept that considers whether a specific system is favored. Thus, a score for favoritism is only applicable to either a pair of systems, or considering one fixed system against all other systems. However, it does not work by considering all pairs of systems at once. Stated differently, we compute Favi Score $\Phi$ based on an evaluation setting $\mathcal{E}$ for a fixed pair of systems. $\Phi$ can be aggregated for one system to determine whether the system is generally favored by a metric in comparison to all other systems. This lies in contrast to performance measure scores, e.g.\ based on correlation, that can be computed over an evaluation setting that contains all pairs of systems.

% \input{algo/phi}

% \paragraph{Computation of the Favi-Score. }~\label{para:algo1}

% In Algorithm~\ref{algo:faviscore} we show the pseudocode how to compute the Favi-Score for two generative systems $\pi_a$ and $\pi_b$, a human preference rating $\mathcal{R}^H$ and an automated preference rating $\mathcal{R}^A$. For each test sample $t$ from a test set $\mathcal{T}$, we compute the corresponding outputs of the two generative systems $\pi_a(t)$ and $\pi_b(t)$, and the human and metric preference ratings $\mathcal{R}^H(\pi_a(t), \pi_b(t))$ and $\mathcal{R}^A(\pi_a(t), \pi_b(t))$, respectively. Each rating is either "+", if the output of $\pi_a$ is preferred, or "-", if the output of $\pi_a$ is preferred, or "=", if both outputs are assessed as of equal quality. The confusion matrix $C \in \mathbb{N}^{3 \times 3}$ counts the number of co-occurrence of the human rating and metric rating, e.g., how often the human rating returns "-" and the metric rating returns "+". The outcome counts $d  \in \mathbb{N}^{3}$ counts the outcomes according to the human ratings (lines 6-10). Finally, $\bm{\mu}$ is computed by normalizing the columns of $C$ (lines 12-13), and the outcome vector $\bm{p}$ is computed by normalizing $d$ (lines 14-15). Finally, the Favi-Score $\Phi$ is computed from $p$ and $\mu$ (line 16), according to Definition \ref{def:faviscore}. 

% %We use a trivial mapping "index" of these ratings $\{+, =, -\}$ to indices in $\{1, 2, 3\}$ to lateron access elements of vectors and matrices. 

% %Then we compute the confusion matrix C, which counts in each of its entries how many test samples have the corresponding human and metrics ratings (line xx ). In addition, we compute the outcome counts $d$ for the human ratings (line xx). 

% %Using C, we can compute the mixture matrix $\mu$ by normalizing C with its column sum (line xx), and we can compute the outcome distribution $p$ from $d$ by normalizing over the sum of entries in $d$. 

% %Finally, we compute the Favi-Score $\Phi$ from $p$ and $\mu$ (line xx), according to Definition \ref{def:faviscore}. 

\section{Alternative Margins}
The definition of the derived preference rating from a scalar in definition~\ref{def:derived_metric} has the issue that for trained metrics based on neural networks, it almost never yields any draws. In the above experiments this leads to low sample-level sign accuracy scores as there all the draw cases lead to mistakes. The main reason is that neural network based metrics return real values, which is almost impossible to return the exact same number for two different inputs. Thus, we also report the experimental results for the following definition of a derived metric.

\begin{definition}[Margin Derived Metric]
\label{def:derived_metric_eps}
    Let $\epsilon_l, \epsilon_r \in \mathbb{R}$ represent two margins. Then the \textbf{margin derived preference metric} $\mathcal{M}$ of a given scalar metric $\mathcal{M}_{s}$ is defined as
    \small
    \[
        \mathcal{M}_{\epsilon}(i, o_1, o_2) =
        \begin{cases}
            + & \mathcal{M}_{s}(i, o_1) > \mathcal{M}_{s}(i, o_2) + \epsilon_l \\
            = & \textit{otherwise} \\
            - & \mathcal{M}_{s}(i, o_1) < \mathcal{M}_{s}(i, o_2) - \epsilon_r \\
        \end{cases}
    \]
\end{definition}

Thus, with the margins the difference between the two ratings needs to be larger than some margin in order to not be counted as a draw. This makes it more likely to observe draws. 

To simulate a scenario where we have a higher sample-level sign accuracy. For this, we optimize the margins $\epsilon_l, \epsilon_r \in \mathbb{R}$ such that the diagonal of $\mu$ is maximised. 

For the experiments, we require two types of ratings: preference ratings made by humans $\mathcal{M}^H$, and metric ratings for the error-prone ratings $\mathcal{M}^A$. We collect this data for three types of domains: Conversational Dialogue Systems, Automated Text Summarization, and Machine Translation. 

Since most metrics return a scalar value, we need to transform them into a preference rating, which is done as follows:

\begin{definition}[Scalar Metric]
    We call real valued functions of inputs and outputs \textbf{scalar metrics}:
    $\mathcal{M}_s: \mathcal{I} \times \mathcal{O} \rightarrow \mathbb{R}$.
\end{definition}


A preference metric can be constructed from a scalar metric as follows:
\begin{definition}
\label{def:derived_metric}
    The \textbf{derived preference metric} $\mathcal{M}$ of a given scalar metric $\mathcal{M}_{s}$
    is defined as
    \small
    \[
        \mathcal{M}(i, o_1, o_2) =
        \begin{cases}
            + & \mathcal{M}_{s}(i, o_1) > \mathcal{M}_{s}(i, o_2) \\
            = & \textit{otherwise} \\
            - & \mathcal{M}_{s}(i, o_1) < \mathcal{M}_{s}(i, o_2) \\
        \end{cases}
    \]
\end{definition}



\subsection{Dialog System Data Collection}
For the Dialog domain, we used the data provided by~\cite{deriu-etal-2023-correction}. It consist of 1000 outputs by 5 dialogue systems in the ParlAI framework~\cite{miller2017parlai}, on the BlendedSkillTask (BST)~\cite{smith-etal-2020-BST}. The setting is that for 1000 static contexts, each of the 5 systems generates the next utterance, and the human reference was used as the 6-th system. Then, they used five different metrics from the DialEval framework by~\cite{yeh2021comprehensive} to rate each output. Since the metrics are trained scalar metrics, we 
%\begin{itemize}[noitemsep,topsep=0pt]
%    \item \textbf{Blenderbot 1.0 - 400distill (BL400distill)}. BlenderBot 1.0~\cite{shuster2022blenderbot} is a transformer-based encoder-decoder bot trained on the Blended Skill Task (BST) data~\cite{smith-etal-2020-BST}. 
    %\item \textbf{Blenderbot 2.0 - 3B Params (BL2-3B)}. The BlenderBot 2.0 extends Blenderbot 1.0 with internet access~\cite{komeili2022BB2internet} and a long-term memory~\cite{xu2022BB2beyond}. 
    %\item \textbf{DialoGPT}. DialoGPT~\cite{zhang2020dialogpt} is a decoder-only dialogue system that fine-tunes GPT-2~\cite{radford2019gpt2} on the Reddit dataset proposed by the DialoGPT authors.
    %\item \textbf{PolyEncoder}. The PolyEnocder~\cite{Humeau2020Poly-encoders} is a retrieval based dialogue system, which selects the most suitable response from a set of candidates. 
    %\item \textbf{SeekerDial3B}. SeekerDial~\cite{shuster2022seeker} improves on the internet search proposed in BlenderBot 2.0
%\end{itemize}

We used ParlAI to generate the response of each of the dialogue systems for 1000 static contexts from the Blended Skill Task (BST) test set. From this set, we selected 50 contexts, and generated all pairwise outputs between all 5 dialogue systems and the human reference. That is, for each context, there are 15 pairs of outputs to be rated. 

We let workers on Amazon Mechanical Turk~\footnote{\url{https://www.mturk.com}} perform a preference rating. That is, for each pair of output, the workers decided, which output is more appropriate. Figure~\ref{fig:dial_ann} shows the annotation tool. Each sample was annotated by three workers. Each worker is payed 15 cents per annotation, and at a rate of 1.5 annotations per minute on average, they achieve a wage of 12\$ per hour. We used workers with the Master status and restricted their geographic location to English-speaking countries (USA, UK, Canada, Ireland, and Australia). In Figure~\ref{fig:dial_ann_instr} shows the instructions given to the annotators. The annotations are ratings on the overall adequacy of the utterances. Since each sample is annotated by three different workers, we aggregate the ratings using the MACE~\cite{hovy2013mace} software, which computes a trustworthiness score for each annotator and generates a weighted average to get the final label. Note that this annotation scheme directly yields preference ratings according to our framework.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/DialAnn.png}
    \caption{Screenshot of the Dialogue Annotation Tool.}
    \label{fig:dial_ann}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/DialAnnInstr.png}
    \caption{Screenshot of the Instruction of the Dialogue Annotation Tool.}
    \label{fig:dial_ann_instr}
\end{figure}

In order to generate the metric ratings, we used the DialEval framework by~\cite{yeh2021comprehensive}, which integrates a large pool of metrics. We selected five metrics that were easy to setup and achieved decent correlations to human judgments in the evaluation by~\cite{yeh2021comprehensive}. Since the metrics return scalar values for each sample, we create preference ratings as suggested in Definition~\ref{def:derived_metric}. Since the scalar metrics yield real numbered values, there are almost no cases where the derived preference rating yields a draw. 

\subsection{Summarization Data Collection}
For the Summarization domain, we use the data provided by the SummEval framework~\cite{fabbri2021summeval}. It contains data from the Dailymail/CNN dataset~\cite{nallapati2016abstractive}, which contains a test set of 11k samples. The SummEval framework contains the outputs of 23 summarization systems (for a detailed description of these systems, we refer the reader to Section 3.2 of~\cite{fabbri2021summeval}). For 16 of the 23 summarization systems, the authors let 100 generated outputs be rated by three experts on the four characteristics: fluency, consistency, coherence, and relevance. Since these ratings are on a Likert-scale, we transformed those ratings into preference ratings by averaging the three ratings per sample, and applying the transformation proposed in definition~\ref{def:derived_metric}. 

We chose 7 automated metrics based on their popularity and ease of setup. We applied the SummEval framework to generate the automated ratings for each of the 16 summarization systems on the full test set. Analogous to above, we converted the scalar ratings to pairwise ratings by applying definition~\ref{def:derived_metric}. 

==> tables/conf_mat_em.tex <==
\begin{tabular}{|c||c | c| c |} \hline
     &  + & = & - \\ \hline 
    600 & 360 &  \cellcolor{green!25}180 &  \cellcolor{green!25}60 \\ \hline
    100 & \cellcolor{blue!25}20 & \textcolor{red}{39} &  \cellcolor{green!25}\textcolor{red}{41} \\ \hline
    300 &  \cellcolor{blue!25}90 & \cellcolor{blue!25} 90 & 120 \\ \hline \hline
     & 470 &  309 & 221 \\ \hline
\end{tabular}

==> tables/conf_mat_pm.tex <==
\begin{tabular}{|c||c | c| c |} \hline
     &  + & = & - \\ \hline 
    600 & \textcolor{red}{359} &  \cellcolor{green!25}180 &  \cellcolor{green!25}\textcolor{red}{61} \\ \hline
    100 & \cellcolor{blue!25}20 & 40 &  \cellcolor{green!25}40 \\ \hline
    300 &  \cellcolor{blue!25}90 & \cellcolor{blue!25} 90 & 120 \\ \hline \hline
     & 469 &  310 & 221 \\ \hline
\end{tabular}

==> tables/confusion_matrix.tex <==
\begin{tabular}{|c||c | c| c |} \hline
     &  + & = & - \\ \hline 
    600 & 360 &  \cellcolor{green!25}180 &  \cellcolor{green!25}60 \\ \hline
    100 & \cellcolor{blue!25}20 & 40 &  \cellcolor{green!25}40 \\ \hline
    300 &  \cellcolor{blue!25}90 & \cellcolor{blue!25} 90 & 120 \\ \hline \hline
     & 470 &  310 & 220 \\ \hline
\end{tabular}

==> tables/confusion_matrix_v2.tex <==
\begin{tabular}{|c||c | c| c | c |} \hline
     &  + & = & - & \\ \hline 
    600 & 360 &  \cellcolor{green!25}180 &  \cellcolor{green!40}60 & + \\ \hline
    100 & \cellcolor{blue!25}20 & 40 &  \cellcolor{green!25}40  & = \\ \hline
    300 &  \cellcolor{blue!40}90 & \cellcolor{blue!25} 90 & 120 & - \\ \hline \hline
     & 470 &  310 & 220 & \\ \hline
\end{tabular}

==> tables/correlation_full.tex <==
%\multicolumn{ 5 }{c}{SummEval Relevance} \\ \hline
\begin{tabular}{|l|l|l|l|}
    \hline
    Metric & SplAcc & SysAcc & Avg$~\Phi$ \\ \hline
    \multicolumn{ 4 }{c}{SummEval Relevance} \\ \hline
    bert\_score & 0.337 & 0.625 & 0.260 \\ \hline
    blanc & 0.336 & 0.500 & 0.370 \\ \hline
    cider & 0.264 & 0.417 & 0.390 \\ \hline
    rouge & 0.317 & 0.550 & 0.320 \\ \hline
    s3 & 0.327 & 0.592 & 0.300 \\ \hline
    summaqa & 0.324 & 0.567 & 0.310 \\ \hline
    supert & 0.317 & 0.517 & 0.450 \\ \hline
    \multicolumn{ 4 }{c}{SummEval Coherence} \\ \hline
    bert\_score & 0.307 & 0.533 & 0.440 \\ \hline
    blanc & 0.303 & 0.417 & 0.510 \\ \hline
    cider & 0.265 & 0.383 & 0.500 \\ \hline
    rouge & 0.302 & 0.483 & 0.460 \\ \hline
    s3 & 0.305 & 0.483 & 0.465 \\ \hline
    summaqa & 0.307 & 0.467 & 0.480 \\ \hline
    supert & 0.305 & 0.433 & 0.495 \\ \hline
    \multicolumn{ 4 }{c}{SummEval Consitency}\\ \hline
    bert\_score & 0.140 & 0.583 & 0.150 \\ \hline
    blanc & 0.163 & 0.533 & 0.350 \\ \hline
    cider & 0.105 & 0.250 & 0.365 \\ \hline
    rouge & 0.144 & 0.383 & 0.225 \\ \hline
    s3 & 0.146 & 0.550 & 0.210 \\ \hline
    summaqa & 0.151 & 0.642 & 0.260 \\ \hline
    supert & 0.137 & 0.533 & 0.400 \\ \hline
    \multicolumn{ 4 }{c}{SummEval Fluency}\\ \hline
    bert\_score & 0.206 & 0.517 & 0.200 \\ \hline
    blanc & 0.208 & 0.458 & 0.410 \\ \hline
    cider & 0.170 & 0.283 & 0.390 \\ \hline
    rouge & 0.192 & 0.417 & 0.220 \\ \hline
    s3 & 0.202 & 0.450 & 0.235 \\ \hline
    summaqa & 0.198 & 0.517 & 0.300 \\ \hline
    supert & 0.195 & 0.475 & 0.445 \\ \hline
    \multicolumn{ 4 }{c}{Dialog}\\ \hline
    deb & 0.322 & 0.600 & 0.204 \\ \hline
    grade & 0.293 & 0.533 & 0.320 \\ \hline
    holistic & 0.247 & 0.267 & 0.540 \\ \hline
    maude & 0.269 & 0.400 & 0.340 \\ \hline
    usl & 0.318 & 0.533 & 0.172 \\ \hline
    \multicolumn{ 4 }{c}{WMT-21}\\ \hline
    C-SPEC & 0.297 & 0.782 & 0.070 \\ \hline
    COMET-DA\_2020& 0.264 & 0.400 & 0.233 \\ \hline
    bleurt-20 & 0.318 & 0.473 & 0.184 \\ \hline
    sentBLEU & 0.304 & 0.436 & 0.180 \\ \hline
    \multicolumn{ 4 }{c}{WMT-22}\\ \hline
    BLEU & 0.396 & 0.444 & 0.129 \\ \hline
    BLEURT-20 & 0.401 & 0.667 & 0.049 \\ \hline
    COMET-22 & 0.291 & 0.611 & 0.080 \\ \hline
    UniTE & 0.419 & 0.722 & 0.079 \\ \hline
    metricx\_xl & 0.412 & 0.778 & 0.069 \\ \hline
\end{tabular}

==> tables/data_tr.tex <==
\begin{tabular}{ l | l | c | c | c | c }
& Data & Metrics & TG System & Human Ratings & Metric Ratings \\\hline
Chatbot & BST & 5 & 6 & 50 & 1k \\
SumEval & CNN/DM & 7 & 11 & 100 & 11k \\
WMT21 & News EN->DE & 4 & 16 & 500 & 1k
\end{tabular}


==> tables/maj_voting.tex <==
\begin{tabular}{ l | c c c c }
Metric & Err & Med. F1 & Med.$\rho$ & Corr. \\ \hline
Chatbot &	0.46 &	0.29 &	0.31 &	$0.42$ \\ 
Summeval Coh. &	0.44 &	0.30 &	0.30 &	$-0.28^{*}$ \\
Summeval Cons. &	0.36 &	0.14 &	0.37 &	$0.25^{*}$ \\ 
Summeval Flu. &	0.45 &	0.20 &	0.32 &	$0.13$ \\
Summeval Rel. &	0.35 &	0.33 &	0.34 &	$-0.06$ \\
WMT21 &	0.63 &	0.30 &	0.40 &	$-0.61^{*}$ \\\hline
\end{tabular}

